Scale functions of space-time changed processes with no positive jumps

The scale functions were defined for spectrally negative L\'evy processes and other strong Markov processes with no positive jumps, and have been used to characterize their behavior. In particular, I defined the scale functions for standard processes with no positive jumps using the excursion measures in Noba(2020). In this paper, we consider a standard process $X$ with no positive jumps and a standard process $Y$ defined by the space-time change of $X$. We express the scale functions of $Y$ using the scale functions of $X$ defined in Noba(2020) and the Volterra integral equation. From this result, we can express the scale functions of some important processes, such as positive or negative self-similar Markov processes with no positive jumps and continuous-state branching processes, using the scale function of spectrally negative L\'evy processes and the Volterra integral equations.

==> style-j.tex <==
%%%%%%    theorems      %%%%%%
\theoremstyle{definition}
\newtheorem{Thm}{'藝}[section]
\newtheorem{Thma}{'藝}
\renewcommand{\theThma}{\Alph{Thma}}
\newtheorem{Thmb}{'藝}
\renewcommand{\theThmb}{\arabic{section}.\Alph{Thmb}}
\newtheorem{Lem}[Thm]{•â'è}
\newtheorem{Prop}[Thm]{–½'è}
\newtheorem{Cor}[Thm]{Œn}
\newtheorem{Ass}[Thm]{‰¼'è}
\newtheorem{Conj}[Thm]{—\'z}
\newtheorem{Def}[Thm]{'è‹`}
\newtheorem{Rem}[Thm]{'}
\newtheorem{Ex}[Thm]{—á}
\newtheorem{Prob}{–â}[section]
\newcounter{Exami}
\newcommand{\Exam}{\noindent \refstepcounter{Exami} $ \boxed{\arabic{Exami}} $ \ }

\newcommand{\Proof}[2][Ø–¾]{
\begin{proof}[{\bf #1}]
#2
\end{proof}
}
\newcommand{\Solution}[2][‰ð]{
\begin{proof}[{\bf #1}]
#2
\end{proof}
}







